Pseudoscalar Higgs Boson Decays into W and Z Bosons Revisited

We examine, in a number of Standard Model extensions, whether the decays $A \to WW/ZZ$ of a neutral pseudoscalar (Higgs) resonance can have branching ratios at the percent level and we determine the possible size of $B(A \to WW/ZZ)$ relative to the respective branching ratios of a scalar boson $H$. The branching ratios of the these decay modes and the total widths $\Gamma_A$, $\Gamma_H$ are computed in the minimal supersymmetric extension of the SM, in a type-II two-Higgs doublet extension (2HDM), in a 2HDM with 4 chiral fermion generations, in a 2HDM with additional heavy vector-like quarks, and in a top-color assisted technicolor model. We find that in the above non-supersymmetric models $B(A \to WW)$ can be about 2%, while $B(A \to ZZ) \lesssim 10^{-3}.$ The ratio $B(A \to WW)/B(H \to WW)$ can be of order 10% in large regions of the parameter space of the models.

==> genloop.tex <==
\unitlength=1bp%

\begin{feynartspicture}(160,80)(2,1)

\FADiagram{(a)}
\FAProp(0.,10.)(6.5,10.)(0.,){/ScalarDash}{0}
\FALabel(3.25,9.18)[t]{$A$}
\FAProp(20.,15.)(13.,14.)(0.,){/Sine}{0}
\FALabel(16.2808,15.5544)[b]{$V$}
\FAProp(20.,5.)(13.,6.)(0.,){/Sine}{0}
\FALabel(16.2808,4.44558)[t]{$V'$}
\FAProp(6.5,10.)(13.,14.)(0.,){/Straight}{1}
\FALabel(9.20801,13.1807)[br]{$F_1$}
\FAProp(6.5,10.)(13.,6.)(0.,){/Straight}{-1}
\FALabel(9.20801,6.81927)[tr]{$F_1$}
\FAProp(13.,14.)(13.,6.)(0.,){/Straight}{1}
\FALabel(14.274,10.)[l]{$F_2$}
\FAVert(6.5,10.){0}
\FAVert(13.,14.){0}
\FAVert(13.,6.){0}

\FADiagram{(b)}
\FAProp(0.,10.)(6.5,10.)(0.,){/ScalarDash}{0}
\FALabel(3.25,9.18)[t]{$A$}
\FAProp(20.,15.)(13.,14.)(0.,){/Sine}{0}
\FALabel(16.2808,15.5544)[b]{$V$}
\FAProp(20.,5.)(13.,6.)(0.,){/Sine}{0}
\FALabel(16.2808,4.44558)[t]{$V'$}
\FAProp(6.5,10.)(13.,14.)(0.,){/Straight}{-1}
\FALabel(9.20801,13.1807)[br]{$F_1$}
\FAProp(6.5,10.)(13.,6.)(0.,){/Straight}{1}
\FALabel(9.20801,6.81927)[tr]{$F_1$}
\FAProp(13.,14.)(13.,6.)(0.,){/Straight}{-1}
\FALabel(14.274,10.)[l]{$F_2$}
\FAVert(6.5,10.){0}
\FAVert(13.,14.){0}
\FAVert(13.,6.){0}
\end{feynartspicture}


